Visual Validation versus Visual Estimation: A Study on the Average Value in Scatterplots

We investigate the ability of individuals to visually validate statistical models in terms of their fit to the data. While visual model estimation has been studied extensively, visual model validation remains under-investigated. It is unknown how well people are able to visually validate models, and how their performance compares to visual and computational estimation. As a starting point, we conducted a study across two populations (crowdsourced and volunteers). Participants had to both visually estimate (i.e, draw) and visually validate (i.e., accept or reject) the frequently studied model of averages. Across both populations, the level of accuracy of the models that were considered valid was lower than the accuracy of the estimated models. We find that participants' validation and estimation were unbiased. Moreover, their natural critical point between accepting and rejecting a given mean value is close to the boundary of its 95% confidence interval, indicating that the visually perceived confidence interval corresponds to a common statistical standard. Our work contributes to the understanding of visual model validation and opens new research opportunities.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> text/fig-valinflection.tex <==
\begin{figure}
 \centering
 \includegraphics[width=0.8\columnwidth]{val_inflection}
 \caption{Histogram of the individual critical points of accepting a given value for the volunteered population in the validation task (absolute deviation). The green line indicates the statistical 95\% CI.}
 \label{fig:val_inflection}
\end{figure}

==> text_initialsubmission/fig-errorcomp.tex <==
\begin{figure}
    \centering
    \begin{subfigure}[t]{0.8\columnwidth}
         \centering
         \includegraphics[width=0.8\columnwidth]{val_est_comp_normal}
         \caption{Volunteered population.}
         \label{fig:comp_normal}
     \end{subfigure}
    
     \begin{subfigure}[t]{0.8\columnwidth}
         \centering
         \includegraphics[width=0.8\columnwidth]{val_est_comp_prolific}
         \caption{Crowdsourced population.}
         \label{fig:comp_prolific}
     \end{subfigure}
        \caption{Validation and estimation accuracy for both populations (absolute deviation). Blue line: Cumulative distribution for the estimation errors. Orange line: Logistic regression for the validation acceptance. Green line: Statistical 95\% CI.}
        \label{fig:comp}
\end{figure}

==> text_initialsubmission/fig-esterror.tex <==
\begin{figure}
 \centering
 \includegraphics[width=0.8\columnwidth]{est_error}
 \caption{Histogram of the deviations of the drawn lines in the estimation tasks for both populations.}
 \label{fig:est_error}
\end{figure}

==> text_initialsubmission/fig-valerror.tex <==
\begin{figure}
 \centering
 \includegraphics[width=0.8\columnwidth]{val_error}
 \caption{Acceptance rate of the shown lines in the validation tasks (absolute deviation) of the volunteered population. Yellow line: The raw percentages per deviation. Orange line: The logistic regression of the yellow line's data. Green line: Statistical 95\% CI.}
 \label{fig:val_error}
\end{figure}

==> text_initialsubmission/fig-valerrorcomp.tex <==
\begin{figure}
 \centering
 \includegraphics[width=0.8\columnwidth]{val_error_comp}
 \caption{Comparison of the logistic regressions for the acceptance rates of positive and negative deviations of the volunteered population. Green line: statistical 95\% CI.}
 \label{fig:val_error_comp}
\end{figure}

==> text_initialsubmission/fig-valinflection.tex <==
\begin{figure}
 \centering
 \includegraphics[width=0.8\columnwidth]{val_inflection}
 \caption{Histogram of the individual critical points of accepting a given value for the volunteered population in the validation task (absolute deviation). The green line indicates the statistical 95\% CI.}
 \label{fig:val_inflection}
\end{figure}

==> text_initialsubmission/intronotes.tex <==
Model validation is the process of checking that a given model result is a good fit to the data. This is needed e.g., in meteorology for data assimilation. Such models are, for example, regressions that are often used in many applications, e.g. in biology, finance, or meteorology, to assess the data patterns (is data stationary or is there a trend?), identify relationships bettween variables (relationship of two variables) or to impute missing values. \textit{(From wiki: Linear regression plays an important role in the subfield of artificial intelligence known as machine learning. The linear regression algorithm is one of the fundamental supervised machine-learning algorithms due to its relative simplicity and well-known properties.)} This model verification can be done computationally or visually. Model validation statistics are often insufficient to fully describe the underlying data and to check the model quality~\cite{Matejka.2017} \textit{TODO reference to statistics of linear models. State why!!} Only humans can verify the model result, its properties beyond statistics and spot additional patterns or data semantics. Thus, it is essential in practise to validate computed models not only through statistical tests, but also visually to ensure that they are accurate and reliable. 

Automatic model selection not possible or not optimal
Looks Good To Me: Visualizations As Sanity Checks
deceptive potential of graphics
Seeing What You Believe or Believing What You See? Belief Biases Correlation Estimation
Outlier detection and rejection in scatterplots
Misinformed by visualizations
fitting bell curves to visualizations
visualization mirages



Model results to be validated are generated by estimation. This estimation can be done computationally (e.g., calculating parameters of linear regression) or visually (by visual aggregation). The results of computational estimation are shown to the user for visual validation or are validated by computer. As stated above, computational validation is not sufficient and visual validation is needed. Alternative model result generation is visual estimation. For example for simple but generalizable models of linear regression to the constant, an average can be estimated visually~\cite{Gleicher.2013, Hong.2022, Yuan.2019}, which is also called visual aggregation.

Ideally the results of visual estimation and visual validation lead to the same: a proper model result. In theory, this should be the case because both processes aim to accurately represent the underlying data generating process.

Despite the importance of visual model validation, there has been relatively little research in this area. Most of the research in the perception of statistical modeling has focused on model estimation~\cite{Correll.2017, Gleicher.2013, Hong.2022, Rensink.2010, Xiong.2022, Yuan.2019}. To our knowledge, no previous studies have specifically investigated the ability of individuals to visually validate statistical models. 

\textit{TODO More related work needed: visualization and visual analytics of modelling, model results, e.g. recent surveys etc. Basically saying visualization, interction, VA creating models, showing models, model results -- there is a lot. The visual model validation cognition, process, etc. not.}

Our work fills this gap in the literature by answering the following research questions:

\begin{itemize}
    \item RQ1: Are people able to visually validate statistical models?
    \item RQ2: What is the performance in terms of accuracy compared to model estimation?
\end{itemize}

We decided to use a linear regression to a constant - simple but generalizable model that is commonly used in applications - as a starting point for our investigation of individuals validation capability. The average height of points in scatterplots describes a linear regression on a constant that summarises the underlying data and provides a simplified representation of its central tendency. The reduced number of parameters in this simplified model allows us to have better control over experimental conditions and statements. Even though the complexity of statistical models can be increased at will, the constant model of the mean allows meaningful results. Furthermore, literature already exists that examines visual average estimation in scatterplots to which we can relate~\cite{Gleicher.2013, Hong.2022, Yuan.2019}.

We conducted a user study to answer our research questions. In the between-subjects setting, participants either had to validate a particular line in a scatterplot in relation to the average height of the dots (\cref{fig:scat_line}) or estimate it by their own (\cref{fig:scat_init}). Conducting the study with two different populations showed to the same results: People are more accurate at estimating models than at validating them. The findings suggest that the perceptual process of validation is more challenging and needs more effort to perform. Furthermore, the critical point between accepting and rejecting a line is pretty close to the boundary of the 95\% confidence interval of the true mean value, which gives evidence that the visual perceived confidence interval corresponds to the statistical confidence interval.

%Sanity checks: For large and complex datasets, visualizations of distributions work as “sanity checks” by providing evidence that the underlying data are reasonably free of flaws such as missing values or excessive noise that might affect later analysis, and by informing hypotheses about interactions and relationships among variables. Sanity checks also build trust in the underlying data processes. These sanity checks assume that data flaws produce characteristic and legible visual signatures in visualizations.

%What for: Quote from Black hat \cite{correll2017black}: "There are three avenues of future work related to black hat vis.
%The first is taxonometric: we should enumerate the ways that visualizations can deceive or mislead. The examples presented in this paper, and in other works, are a fraction of this enormous space. The second avenue is empirical: rather than taking it on faith that these attacks are or are not effective to our target audiences, we should collect empirical evidence on the size and reliability of these effects (as per [6, 18]). The last avenue is detection and prevention  of bad behavior: “white hat vis,” using our analogy. There are many automated tools for generating and interacting with visualizations. To encourage the responsible use of these tools, we need to develop methods for detecting and correcting for their misuse. This “defensive design” could take the form of automated assistants (such as systems to detect and correct suboptimal color maps [20]), or could exist as codified design principles and best practices. However, at a minimum, we ought to bake in more supervision and guidance into visual analytics systems, through smart defaults, automated feedback, and explicit warnings to users and consumers of visualizations. "


%Mirages paper: Dirty data and deceptive design practices can undermine, invert, or invalidate the purported messages of charts and graphs.  These failures can arise silently: a conclusion derived from  a particular visualization may look plausible unless the analyst looks closer and discovers an issue with the backing  data, visual specification, or their own assumptions. We term  such silent but significant failures visualization mirages.

%Sanity checks: For large and complex datasets, visualizations of distributions work as “sanity checks” by providing evidence that the underlying data are reasonably free of flaws such as missing values or excessive noise that might affect later analysis, and by informing hypotheses about interactions and relationships among variables. Sanity checks also build trust in the underlying data processes. These sanity checks assume that data flaws produce characteristic and legible visual signatures in visualizations.

%What for: Quote from Black hat \cite{correll2017black}: "There are three avenues of future work related to black hat vis.
%The first is taxonometric: we should enumerate the ways that visualizations can deceive or mislead. The examples presented in this paper, and in other works, are a fraction of this enormous space. The second avenue is empirical: rather than taking it on faith that these attacks are or are not effective to our target audiences, we should collect empirical evidence on the size and reliability of these effects (as per [6, 18]). The last avenue is detection and prevention  of bad behavior: “white hat vis,” using our analogy. There are many automated tools for generating and interacting with visualizations. To encourage the responsible use of these tools, we need to develop methods for detecting and correcting for their misuse. This “defensive design” could take the form of automated assistants (such as systems to detect and correct suboptimal color maps [20]), or could exist as codified design principles and best practices. However, at a minimum, we ought to bake in more supervision and guidance into visual analytics systems, through smart defaults, automated feedback, and explicit warnings to users and consumers of visualizations. "


%Mirages paper: Dirty data and deceptive design practices can undermine, invert, or invalidate the purported messages of charts and graphs.  These failures can arise silently: a conclusion derived from  a particular visualization may look plausible unless the analyst looks closer and discovers an issue with the backing  data, visual specification, or their own assumptions. We term  such silent but significant failures visualization mirages.



With our work, we are contributing to a better understanding of visual model perception and opening up a new area of research that holds many interesting aspects for further investigation.

\textbf{Contributions/results}
\begin{itemize}
    \item statistical CI = visually perceived CI
    \item symmetry: low=high
    \item prolific vs volunteers: same main results, slightly better for volunteers
    \item estimation better accuracy than validation
    \item personal difference: strong difference
    \item estimation errors normally distributed - corresponds to the linear regression model assumption
    \item validation errors normally distributed
    \item influence of box on validation errors: box higher acceptance
    \item JND switch corresponds to 95\% CI
\end{itemize}



==> text_initialsubmission/sec-abstract.tex <==
% Edit this file
\abstract{%
  We investigate the ability of individuals to visually validate statistical models in terms of their fit to the data. 
  % , which is needed to check model quality. 
  % However, w
  While visual model estimation has been studied extensively,
  % –- especially for averages -– 
  visual model validation remains under-investigated. It is unknown how well people are able to visually validate models, and how their performance compares to visual and computational estimation. As a starting point, we conducted a study across two populations (crowdsourced and volunteers). Participants had to both visually estimate (i.e, draw) and visually validate (i.e., accept or reject) the frequently studied model of averages. 
  Across both populations, the level of accuracy of the models that were considered valid was lower than the accuracy of the estimated models.
  %Across both populations, participants were more accurate at estimating models (i.e., fitting a model to the data) than validating them (i.e., judging models as correct or incorrect). 
  We find that participants' validation and estimation were unbiased by the characteristics of the data (e.g., data distributions). Moreover, their natural critical point between accepting and rejecting a given mean value is close to the boundary of its 95\% confidence interval, indicating that the visually perceived confidence interval corresponds to a common statistical standard.
  %This finding indicates that the visually perceived confidence interval corresponds to the statistical confidence interval for average validation across populations. 
  Our work contributes to the understanding of visual model validation and opens new research opportunities.}
  
  %Overall, our results suggest that there exists differing cognitive processes affecting accuracy when estimating versus validating models over data, indicating that the design of model visualizations should consider people’s inherent ability to estimate models.
% 
% 
%   In today's data-driven world, experts use visual validation to check their model's quality, while the general public uses visual validation to consume news media visualizations, e.g., to contextualize trends or inform policies. Despite this prevalence, our understanding of an individual's ability to accurately validate models is under-investigated, while visual model \textit{estimation} has been studied extensively. As a starting point to address this gap, we present a study conducted across two populations
%   
    %Full paper version
% \abstract{%
%   % ashley's updated version
%   We investigate the ability of individuals to visually validate statistical models in terms of their fit to the data.  Visual validation is needed in practice by experts for checking their model’s quality, and by the general public for consuming news media visualizations and model results that affect policies. However, while visual model estimation, so-called "regression-by-eye," has been studied extensively – especially for averages – visual model validation remains under-investigated. As a result, it is unknown how well people are able to visually validate models, and how their performance compares to visual and computational estimation. As a starting point in answering this question, we conducted a study across two populations (crowdsourced and volunteers) in which participants had to both visually estimate (i.e. draw) and visually validate (i.e. accept or reject) a model over data. We chose the frequently studied model of averages, i.e. regression to a constant, in order to easily compare against prior research in model estimation. Across both participant populations, our results indicate that people are more accurate at estimating models (i.e., fitting a model to the data) than validating them (i.e. judging models as correct or incorrect). We find that a human's natural critical point between accepting and rejecting a given mean value is close to the boundary of the 95\% confidence interval, even when no confidence interval is shown in the visualization. This provides evidence that the visually perceived confidence interval corresponds to the statistical confidence interval for average estimation across populations. Overall, our results suggest that there exists differing cognitive processes affecting accuracy when estimating versus validating models over data, indicating that the design of model visualizations should consider people’s inherent ability to estimate models. We discuss the implications of our study results in model interpretability, decision-making, and how future work can be done to generalize across more robust models.}
  
  % Daniel's & Tatiana's version from march 19
%   We investigate the ability of individuals to visually validate statistical models in terms of their fit to the data.  Visual validation is needed in practice by experts for checking model quality and by general public for detecting possible deceipt in the visualization or model result. While visual model estimation, so-called "regression-by-eye", has been studied extensively, especially for averages, visual model validation is still under-investigated. It is unclear how well people are able to visually validate models and how it compares to visual estimation and to computational estimation. As a starting point analysing this question, we chose simplest possible model: estimating averages, i.e., regression to a constant. In our two studies with two populations (crowdsourcing and volunteers), both across expertise, age and backgrounds, half of participants had to visually estimate and half had to visually validate average value estimation. The results indicate that people are more accurate at estimating models than validating them. Interestingly, although there was no visualization of the confidence interval, the human's natural critical point between accepting and rejecting a given mean value is close to the boundary of the 95\% confidence interval. This gives evidence, that the visual perceived confidence interval corresponds to the statistical confidence interval for average estimation across populations. Our findings indicate, that people are able to visually validate statistical models of averages and that visualization designers and practitioners cannot deceipt people with wrong average visualizations. A generalization of our results, the perceptual mechanisms of visual validations, other visualization designs, and visual validation  of other models, will be studied in future.}

%old Friday 17.3.:  We investigate the ability of individuals to visually validate statistical models in terms of their fit to the data. Fitting averages, i.e. a regression to a constant  is a base example. Visual validation is needed in practice because statistical tests alone are not sufficient to determine the quality of a computed model. While visual model estimation, i.e. the visual generation of a model result, has been studied extensively, especially for averages, there is almost no research on visual model validation. We conducted a user study of validating computed averages in scatterplots to find out how accurate people are in validating models and how their performance compares to model estimation. The results indicate that people are more accurate at estimating models than validating them, and the critical point between accepting and rejecting a given mean value is close to the boundary of the 95\% confidence interval of the true mean value. This gives evidence, that the visual perceived confidence interval corresponds to the statistical confidence interval. Our findings contribute to a better understanding of visual model perception and open up new avenues for further investigation. 


==> text_initialsubmission/sec-conclusion.tex <==
\section{Conclusion}
\label{sc:conclustion}

Our empirical user study with two different populations investigated the difference between visual model estimation and visual model validation by using the average value in scatterplots as a baseline. Our findings suggest that 
%visual model estimation is generally more accurate than visual model validation and that both processes are unbiased. Moreover, people's natural critical point between accepting and rejecting a given mean is close to the boundary of the statistical 95\% confidence interval. 
visual model validation accepts models that are less accurate than those that are estimated visually. The acceptance level is similar to the common statistical standard 95\% confidence interval. 
Our study provides valuable insights into how humans process statistical information and identifies limitations and potential aspects for future research. 

% I am not sure that either of these follow from what we have found!
% Overall, this study highlights the importance of combining statistical methods with human perception to improve model validation in various domains. Our results are useful for both domain experts and general public.

==> text_initialsubmission/sec-futurework.tex <==
\section{Limitations and Future Work}
\label{sc:fw}

% Obtaining similar results for different populations indicates the generalizability of our findings with respect to populations. Nevertheless, as a starting point for further research on visual validation, we focused on a specific type of data, visualization, and model, so the generalizability with respect to these aspects remains to be proven.

% Furthermore, we do not yet know anything about the perceptual mechanisms involved in visual model validation. It would also be interesting to explore the influence of visual encoding and data patterns (e.g., outliers, shapes, etc.).

%We recruited two participant groups for our study: The first from the crowdsourced platform Prolific, and the second from a university's student mailing list. 
%This study aimed to investigate visual model validation in the context of modeling the average for data shown in scatterplots \remco{I don't fully understand this sentence}. 
%The participants in this study were not experts in data visualization or statistics, making them representative of the general public rather than domain experts who regularly conduct visual model validation in a workplace setting.
The participants in this study were non-experts in data visualization or statistics, making them not representative of domain experts.
Although our findings are statistically sound, since we chose to focus on a specific type of data, visualization, and model as a starting point to understand visual model validation, the generalizability of our results regarding these aspects remains to be established.
%By choosing to focus on a specific type of data, visualization, and model as a starting point in understanding visual model validation, the generalizability of our results with respect to these aspects remains to be proven.

Furthermore, we need to investigate the perceptual mechanisms involved in performing visual model validation, and how they compare to the mechanisms when performing visual model estimation. It would also be interesting to explore the influence of visual encoding and data patterns (e.g., outliers, shapes). By doing so, we could derive design guidelines for model visualizations that mitigate perceptual biases in visual validation (e.g., the work by Hong et al.\cite{Hong.2022}). As part of these design guidelines, we plan to provide prescriptive instructions in future work on when and how visualizations should include pre-drawn models fitted to data.

% \textbf{future work}

% \begin{itemize}
%     \item influence of visual encoding
%     \item study of perception mechanisms
%     \item generalization to other regressions e.g. trends, and other type of data e.g. time series (trend for estimation proven to work well, as well as averages, so we could assume this could be possible)
%     \item influence of visual patterns e.g. outliers, etc.
%     \item validation of own estimated models
% \end{itemize}



==> text_initialsubmission/sec-intro.tex <==

In today's data-driven world, individuals with a range of statistical expertise are tasked with visually validating statistical models fitted to data for a variety of purposes. Domain experts (often with statistical expertise) use visual validation to quickly determine whether a particular model is a good fit to the underlying data (e.g., meteorologists validating a model for assimilation). Similarly, the general public (who may not have statistical expertise) also use visual model validation when consuming news media visualizations, e.g., to become informed about changes of COVID-19 cases over time (such as using a 14-day moving average model visualization\cite{dansana2020global}). 
%For example, statistical model visualizations fitted to data were regularly shown to inform the general public of how COVID-19 cases were changing over time (e.g., using a 14-day moving average model visualization~\cite{dansana2020global}). 

To perform model validation, an individual checks that a given model result is a good fit to the data. This model verification can be done computationally or visually; however, statistics computed to validate models are often insufficient to fully describe the underlying data and model's quality\cite{Matejka.2017}. 
% Consequently, humans utilize perception to verify the model's properties beyond statistics, e.g., to spot additional patterns. 
Thus, 
it is essential in practice to validate computed models not only through statistical tests, but also visually to ensure that they are accurate and reliable.

Despite the prevalence of visual model validation\cite{Muehlbacher.2013}, there is markedly little research done to understand viewers' ability % an individual's ability % this isn't per person
to perform these processes.
Instead, most research in the perception of statistical modeling has focused on \textit{model estimation}\cite{Correll.2017, Gleicher.2013, Hong.2022, Rensink.2010, Xiong.2022, Yuan.2019, Yang.2019, Harrison.2014, Kay.2016, Newburger.2022}, that is, the ability of an individual to perceive, draw, or predict a model that is appropriately fitted to the data. While these studies help inform our understanding of experts and non-experts' strengths and limitations in \textit{estimating} models, they do not advise us of an individual's ability to \textit{validate} how well a statistical model fits the data. 
As a result, it is currently unknown how well people validate models in comparison to their estimation ability, how the design of model visualizations should incorporate the strengths and weaknesses of an individual's ability to validate models, and how factors like trust and statistical expertise affect it. 
%For example, whether an individual's trust in a model or data source can result in higher or lower visual validation (i.e. acceptance) in the shown model with respect to the data.

We seek to establish a baseline for understanding the differences between an individual's ability to perform model estimation and validation, as well as to compare against existing literature in visual model estimation\cite{Gleicher.2013, Hong.2022, Yuan.2019}.
As an initial exploration, we chose to use the model of \textit{averages} (mean expected value) in scatterplots. The model of averages is a simple but generalizable model that is widely used in visual analysis~\cite{Demir.2016, Dube.2019} applications and corresponds to the result of a linear regression to a constant that summarises the underlying data and provides a simplified representation of its central tendency.
%The model of averages is a simple but generalizable model that is widely used in visual analysis applications; furthermore, the average value of points in scatterplots corresponds to the result of a linear regression to a constant that summarises the underlying data and provides a simplified representation of its central tendency. The low number of parameters in this model allows us to control experimental conditions and assumptions. 

Using this setting, we compare the visual processes of model validation and estimation and answer the following research questions:
\begin{itemize}[noitemsep, nolistsep]
    %\item \textbf{RQ1}: Are individuals able to accurately and unbiasedly validate statistical models visually (specifically averages)?
    % \item \textbf{RQ1}: Are individuals able to accurately visually validate statistical models (specifically averages) across different data distributions?
    \item \textbf{RQ1}: Are individuals able to perform visual validation consistently and without bias for averages across different data distributions?
    % \item \textbf{RQ2}: How does the accuracy of visual validation compare to the visual model estimation of averages?
    \item \textbf{RQ2}: How does performance in visual validation relate to the accuracy of visual estimation?
\end{itemize}


We conducted a human subjects study with two participant groups to address these research questions. Using a between-subjects study design, participants either had to validate whether a shown line in a scatterplot represents the average value of the dots (\autoref{fig:scat_line}) or had to estimate the average line on their own (\autoref{fig:scat_init}).
% From our study, we found that -- across both participant populations -- people are consistently more accurate at \textit{estimating} a model representing the average value of a scatterplot than at \textit{validating} a pre-fit line in relation the average value.
Our study finds that the participants are consistent and unbiased (i.e. not influenced by data distribution) when deciding the threshold for a model to be accepted as valid. Furthermore, the required level of accuracy for validation was found to be lower than what can be estimated through visual inspection.
%From our study, we found that -- across both participant populations -- people are consistently more accurate at \textit{estimating} a model representing the average value of a scatterplot than \textit{validating} the accuracy of a pre-fit line representing the average value of a scatterplot. 
%Furthermore, 
We find that the critical point between accepting and rejecting a line is close to the boundary of the 95\% confidence interval (CI) of the true mean value (i.e., a common statistical criteria for validity). 
% The implications of our findings are two-fold. 
These results have two major implications.
%First, the higher performance of individuals to perform model estimation over validation suggests that the perceptual process of validation is more challenging. 
First, viewers accept models that are less accurate than they can estimate visually.
Second, individuals' ability to judge a model within the 95\% CI suggests that the visual perceived confidence interval corresponds to a common statistical standard. % the statistical CI. 
% In Section~\ref{ssc:expdesign}, we discuss the setup of our study and our findings in detail. 

%Overall, our work contributes towards a better understanding of visual model validation that is needed by both experts for model checking and by the general public for trust in models shown in media platforms. 
Overall, our work contributes towards a new understanding of how well people can visually validate a model when given data. 
Our study of averages is a simple regression model that provides a baseline for contributing towards this understanding, which opens up future work for generalization beyond scatterplots and the model of averages. 
%For the remainder of this paper, we discuss prior work in the area then describe the protocol and results of our study. From our findings, we distill limitations and future work for the processes of visual model validation and estimation.  



% Model validation is the process of checking that a given model result is a good fit to the data. Such models are, for example, regressions. This model verification can be done computationally or visually. The computed model validation statistics are often insufficient to fully describe the underlying data and to check the model quality~\cite{Matejka.2017}. Only humans can verify the model result, its properties beyond statistics and spot additional patterns. Thus, it is essential in practise to validate computed models not only through statistical tests, but also visually to ensure that they are accurate and reliable.

% In practice, visual model validation is needed both by experts and by general public. Domain experts, e.g., meteorologists need to validate models for data assimilation, or other domains such as biology, or finance. In finance, for example, regression to a constant is used to validate whether the data is stationary or is there a trend, or to identify relationships between variables. At the same time, general public consumes charts with model results, such as results of weather models or economic or health models. Their trust to these model results means to visually validate (i.e., accept) the shown model result with respect to the data.

% Model results to be validated are generated by model estimation. This estimation can be done computationally (e.g., by calculating parameters of a linear regression) or visually (by visual aggregation, doing "regression by eye"~\cite{Correll.2017}). 
% These (either computationally or visually) estimated models are then visualized for validation purposes. Ideally, the results of visual estimation and visual validation lead to the same model result by construction: both processes aim to accurately represent the same underlying data-generating process.

% Despite the importance of visual model validation~\cite{Muehlbacher.2013}, there has been relatively little research in this area in the visualization community. Most of the research in the perception of statistical modeling has focused on visual model estimation~\cite{Correll.2017, Gleicher.2013, Hong.2022, Rensink.2010, Xiong.2022, Yuan.2019, Yang.2019, Harrison.2014, Kay.2016, Newburger.2022}. Our study paves the way to studies investigating the ability of individuals to visually validate statistical models. 

% As a starting point for the exploration of individuals' validation capability, we decided to use the mean (expected value) -- a simple but generalizable model that is commonly used in applications. The average value of points in scatterplots corresponds to the result of a linear regression to a constant that summarises the underlying data and provides a simplified representation of its central tendency. The low number of parameters in this model allows us to control experimental conditions and statements. This model of averages allows us to compare our results with the literature studying visual average estimation in scatterplots~\cite{Gleicher.2013, Hong.2022, Yuan.2019}.

% Using this setting, we compare the visual processes of model validation and estimation and answer the following research questions:
% \begin{itemize}[noitemsep]
%     \item RQ1: Are individuals able to accurately and unbiased visually validate statistical models -- averages?
%     \item RQ2: How does the accuracy of visual validation compare to the visual model estimation of averages?
% \end{itemize}

% We conducted a user study to answer the research questions. In the between-subjects setting, participants either had to validate whether the shown line in a scatterplot represents the average value of the dots (\autoref{fig:scat_line}) or had to estimate the average line on their own (\autoref{fig:scat_init}). Conducting the study twice, each time with a different population showed to the same results: People are more accurate at estimating models than at validating them. Both validation and estimation is unbiased. Further findings suggest that there is no significant difference between the perceptual process of validation and estimation w.r.t. time and difficulty. Interestingly, the critical point between accepting and rejecting a line is close to the boundary of the 95\% confidence interval (CI) of the true mean value. This indicates that the visually perceived confidence interval corresponds to the statistical CI.

% Our work contributes to a better understanding of visual model validation that is needed by experts for model checking and by general public for trust in shown models in mass media. Our study of averages is a simple regression model, that needs to be generalized in future. Thus, it opens up a new area of research that holds many interesting aspects for further investigation.

% \section{Ashley's Intro}

% In today's data-driven world, individuals with a range of statistical expertise are tasked (whether implicitly or explicitly) with visually validating a statistical model fitted to data for a variety of purposes. For example, domain experts -- those typically with high statistical expertise -- must use visual validation to quickly determine whether a particular model is a good fit to the underlying data. Similarly, the general public (those who may not have high statistical expertise) must also use visual model validation when consuming news media visualizations, e.g., to contextualize trends or public policies. For example, statistical model visualizations fitted to data were regularly shown to inform the general public of how COVID-19 cases were changing over time (e.g., using a 14-day moving average model visualization~\cite{dansana2020global}).

% Despite the prevalence of visual model validation~\cite{Muehlbacher.2013}, there is markedly little research done to understand an individual's ability to perform these processes.
% Instead, most research in the perception of statistical modeling has focused on \textit{model estimation}~\cite{Correll.2017, Gleicher.2013, Hong.2022, Rensink.2010, Xiong.2022, Yuan.2019, Yang.2019, Harrison.2014, Kay.2016, Newburger.2022}, that is, the ability of an individual to perceive, draw, or predict a model that is appropriately fitted to the data. While these studies help inform our understanding of experts and non-experts' strengths and limitations in \textit{estimating} models, they do not advise us of an individual's ability to \textit{validate} a pre-fit statistical model to data. 
% As a result, it is currently unknown how well people validate versus estimate models, how the design of model visualizations should incorporate the strengths and weaknesses of an individual's ability to validate models, and how factors like trust and statistical expertise affect model validation.

% To take a step towards understanding the model validation capabilities of individuals, we conducted a large between-subjects study across two participant groups. In the first group, participants were recruited using the crowdsourced platform Prolific, while the second group of participants were recruited from a university's mailing list. For both groups, participants were tasked with (1) estimating (i.e.\ drawing) an accurately fitted statistical model over data shown on a scatterplot, and (2) validating the accuracy (i.e.\ choosing between `correct' or `not correct') of a pre-drawn statistical model over data shown on a scatterplot. To establish a baseline for understanding the differences between an individual's ability to perform model estimation and validation, as well as to compare against existing literature in visual model estimation over scatterplots~\cite{Gleicher.2013, Hong.2022, Yuan.2019}, we chose to use the model of \textit{averages} (mean expected value) for the participants' tasks. Specifically, participants were asked to either draw (estimate) or judge (validate) a line representing the \textit{average height} given the y-values of data points on a scatterplot (as shown in \autoref{fig:scat_line} and \autoref{fig:scat_init}). This average model describes the linear regression on a constant that summarises the underlying data and provides a simplified representation of its central tendency, allowing us to have better control over experimental conditions and assumptions. 

% Given this study and task design, we compare the visual processes and consistency of model validation versus estimation to answer the following research questions (RQs):
% \begin{itemize}[noitemsep]
%     \item RQ1: Are individuals able to visually validate statistical models?
%     \item RQ2: What is the performance in terms of accuracy compared to model estimation?
% \end{itemize}

% From our study, we found that -- across both participant populations -- 
% people are consistently more accurate at \textit{estimating} a model representing the average height of a scatterplot than \textit{validating} the accuracy of a pre-fit line representing the average height of a scatterplot. Furthermore, we found that the critical point between accepting and rejecting a line is significantly close to the boundary of the 95\% confidence interval of the true mean value. The implications of our findings are two-fold. First, the higher performance of individuals to perform model estimation over validation suggests that the perceptual process of validation is more challenging and requires more effort to perform. Second, individuals' ability to judge a model within the 95\% CI suggests that the visual perceived confidence interval corresponds to the statistical confidence interval. In Section~\ref{ssc:expdesign}, we discuss the setup of our study and our findings in detail. 

% ASHLEY STOPPED HERE

% With our work, we are contributing to a better understanding of visual model perception and opening up a new area of research that holds many interesting aspects for further investigation.

% \textbf{Contributions/results}
% \begin{itemize}
%     \item statistical CI = visually perceived CI
%     \item symmetry: low=high
%     \item prolific vs volunteers: same main results, slightly better for volunteers
%     \item estimation better accuracy than validation
%     \item personal difference: strong difference
%     \item estimation errors normally distributed - corresponds to the linear regression model assumption
%     \item validation errors normally distributed
%     \item influence of box on validation errors: box higher acceptance
%     \item JND switch corresponds to 95\% CI
% \end{itemize}


    %Full paper version
% Model validation is the process of checking that a given model result is a good fit to the data. This is needed, e.g., in meteorology for data assimilation. Such models are, for example, regressions that are often used in many applications, e.g. in biology, finance, or meteorology, to assess the data patterns (is data stationary or is there a trend?), identify relationships between variables (relationship of two variables) or to impute missing values. \textit{(From wiki: Linear regression plays an important role in the subfield of artificial intelligence known as machine learning. The linear regression algorithm is one of the fundamental supervised machine-learning algorithms due to its relative simplicity and well-known properties.)} This model verification can be done computationally or visually. Model validation statistics are often insufficient to fully describe the underlying data and to check the model quality~\cite{Matejka.2017} \textit{TODO reference to statistics of linear models. State why!!} Only humans can verify the model result, its properties beyond statistics and spot additional patterns or data semantics. Thus, it is essential in practise to validate computed models not only through statistical tests, but also visually to ensure that they are accurate and reliable. 

% Model results to be validated are generated by estimation. This estimation can be done computationally (e.g., calculating parameters of linear regression) or visually (by visual aggregation). The results of computational estimation are shown to the user for visual validation or are validated by computer. As stated above, computational validation is not sufficient and visual validation is needed. Alternative model result generation is visual estimation. For example for simple but generalizable models of linear regression to the constant, an average can be estimated visually~\cite{Gleicher.2013, Hong.2022, Yuan.2019}, which is also called visual aggregation.

% Ideally the results of visual estimation and visual validation lead to the same: a proper model result. In theory, this should be the case because both processes aim to accurately represent the underlying data generating process.

% Despite the importance of visual model validation, there has been relatively little research in this area. Most of the research in the perception of statistical modeling has focused on model estimation~\cite{Correll.2017, Gleicher.2013, Hong.2022, Rensink.2010, Xiong.2022, Yuan.2019}. To our knowledge, no previous studies have specifically investigated the ability of individuals to visually validate statistical models. 

% \textit{TODO More related work needed: visualization and visual analytics of modelling, model results, e.g. recent surveys etc. Basically saying visualization, interction, VA creating models, showing models, model results -- there is a lot. The visual model validation cognition, process, etc. not.}

% Our work fills this gap in the literature by answering the following research questions:

% \begin{itemize}
%     \item RQ1: Are people able to visually validate statistical models?
%     \item RQ2: What is the performance in terms of accuracy compared to model estimation?
% \end{itemize}

% We decided to use a linear regression to a constant - simple but generalizable model that is commonly used in applications - as a starting point for our investigation of individuals validation capability. The average height of points in scatterplots describes a linear regression on a constant that summarises the underlying data and provides a simplified representation of its central tendency. The reduced number of parameters in this simplified model allows us to have better control over experimental conditions and statements. Even though the complexity of statistical models can be increased at will, the constant model of the mean allows meaningful results. Furthermore, literature already exists that examines visual average estimation in scatterplots to which we can relate~\cite{Gleicher.2013, Hong.2022, Yuan.2019}.

% We conducted a user study to answer our research questions. In the between-subjects setting, participants either had to validate a particular line in a scatterplot in relation to the average height of the dots (\autoref{fig:scat_line}) or estimate it by their own (\autoref{fig:scat_init}). Conducting the study with two different populations showed to the same results: People are more accurate at estimating models than at validating them. The findings suggest that the perceptual process of validation is more challenging and needs more effort to perform. Furthermore, the critical point between accepting and rejecting a line is pretty close to the boundary of the 95\% confidence interval of the true mean value, which gives evidence that the visual perceived confidence interval corresponds to the statistical confidence interval.

% With our work, we are contributing to a better understanding of visual model perception and opening up a new area of research that holds many interesting aspects for further investigation.


==> text_initialsubmission/sec-rw.tex <==
\section{Related Work}
\label{sc:rw}

\paragraph{Visual Model Estimation}

Research on visual model estimation has investigated the concept of ensemble coding, the rapid extraction of visual statistics on distributions of spatial or featural visual information to estimate actual statistics on data\cite{Szafir2016ensemble}. In particular, the estimation of linear regression to a constant, or average estimation, has been extensively studied for scatterplots: Hong et al. explored the influence of a third dimension, encoded by color or size of the dots, on mean estimation\cite{Hong.2022}. They found that people's mean position estimations are biased towards larger and darker dots. Similarly, Gleicher et al. investigated the perception of average dot height in multi-class scatterplots and found that the perceptual process is robust against more points, sets, or conflicting encodings\cite{Gleicher.2013}. Additionally, Yuan et al. found that the visual estimation of averages depends on the visual encoding of the data and that estimation is more accurate in bar charts than in scatterplots\cite{Yuan.2019}. In line with these previous works, this paper uses scatterplots and averages as a baseline for visual model validation research.

Visual estimation of linear trends, e.g., correlations of two-dimensional data, has also been considered from several aspects. Rensink and Baldridge\cite{Rensink.2010} examined the statistical properties at which a correlation can be perceived for data in scatterplots. Rather than statistical properties, Yang et al.\cite{Yang.2019} focused on the visual patterns of data in scatterplots and their effect on the perception of correlations. Their results suggest that visual features, such as bounding boxes, influence people's correlation judgments. Xiong et al.\cite{Xiong.2022} consider the correlation in scatterplots from a data semantics point of view. They found that people estimate the correlation more accurately with generic axis labels than with meaningful labels. Furthermore, people overestimate correlations between variables when they believe the two should have a strong relationship. Comparisons and rankings of different correlation visualizations based on Weber's law showed measurable differences between various designs (with scatterplots being the best) and that the performances differ significantly for positive and negative correlations\cite{Harrison.2014, Kay.2016}. These works support our choice of scatterplots for our study, which allow for extensibility of the studied model in future work. Moreover, their findings influenced our hypotheses and stimuli design (see \autoref{ssc:pilotstudy} and \autoref{sssc:stimulidesign}).



%Visual model estimation has been researched for several types of models\cite{Szafir2016ensemble}. The visual estimation of a linear regression to a constant, i.e., the average estimation, has been studied mainly for scatterplots. 
%% Therefore, we also focus on this model and visualization type. 
%Hong et al.\cite{Hong.2022} investigated the influence of a third dimension, encoded by the color or size of the dots, on the mean estimation. They found that people's estimated mean position is biased in the direction of larger and darker dots. Gleicher et al.\cite{Gleicher.2013} explored the perception of the average height of dots in multi-class scatterplots. The results of their user study indicate that the perceptual process is robust against more points, more sets, or conflicting encodings of the dots. Yuan et al.\cite{Yuan.2019} found that people's visual proxies for extracting averages depend on the visual encoding of the data and that the visual estimation is more accurate for bar charts than for scatterplots. Similar to how these prior works used scatterplots and averages to explore their research questions, we use the same setup to provide a baseline for visual model validation research.

%Visual estimation of linear trends, e.g., correlations of two-dimensional data, has also been considered from several aspects. Rensink and Baldridge\cite{Rensink.2010} examined the statistical properties at which a correlation can be perceived for data in scatterplots. Rather than statistical properties, Yang et al.\cite{Yang.2019} focused on the visual patterns of data in scatterplots and their effect on the perception of correlations. Their results suggest that visual features, such as bounding boxes, influence people's correlation judgments. Xiong et al.\cite{Xiong.2022} consider the correlation in scatterplots from a data semantics point of view. They found that people estimate the correlation more accurately with generic axis labels than with meaningful labels. Furthermore, people overestimate correlations between variables when they believe the two should have a strong relationship. Comparisons and rankings of different correlation visualizations based on Weber's law showed big differences between various designs (with scatterplots being the best) and that the performances differ significantly for positive and negative correlations\cite{Harrison.2014, Kay.2016}. These works support our choice of scatterplots for our study, which allow for extensibility of the studied model in future work. Moreover, their findings influenced our hypotheses and stimuli design (see \autoref{ssc:pilotstudy} and \autoref{sssc:stimulidesign}).
%A comparison and ranking of different correlation visualizations based on Weber's law is provided by Harrison et al.~\cite{Harrison.2014}. Their study showed big differences between various designs (with scatterplots being the best) and that the performances differ significantly for positive and negative correlations. Kay and Heer~\cite{Kay.2016} revise the previous ranking with a refinement of Weber's law based on Bayesian statistics. Despite the adjusted model, the scatterplot still turns out to be the best possible visualization for the perception of correlation.

%Some research exists also for the estimation of more complex models. 
Research has also been conducted on the visual estimation of more complex models. 
For example, Correll and Heer\cite{Correll.2017} investigated people's ability to perform ``regression by eye'' for different types of trends and visualization types. Their results showed that individuals can accurately estimate trends in many standard visualizations; however, both visual features and data features (e.g., outliers) can affect the results. Another study of Newburger et al.\cite{Newburger.2022} focused specifically on fitting bell curves to different visualization types. They found that people are accurate at finding the mean, but tend to overestimate the standard deviation. In our study, we aim to explore whether the findings from these papers also apply to visual validation for less complex models.

%Although we focus on average values in scatterplots, the insights from the related papers are important for future extensions of our work to other visual encodings and models.

\paragraph{Visual Model Validation}

%There exists little literature on visual model validation. 
The literature on visual model validation is currently limited. 
Correll et al.\cite{Correll.2018} evaluated scatterplots, histograms and density plots as means to support data quality checks. Their findings suggest that problems arise as soon as overplotting occurs, which informed the design of the scatterplots in our study.
%Their results for scatterplots show that problems occur as soon as overplotting occurs, so we only use data without overplotting.

%Machine learning is an area in which visual model validation is important. 
Visual model validation is particularly significant in the field of machine learning. The survey by Chatzimparmpas et al.\cite{Chatzimparmpas.2020} provides an overview of how visualization is currently used to interpret machine learning models. Mühlbacher and Piringer~\cite{Muehlbacher.2013} present a partition-based framework for creating and validating regression models that combines the use visualizations with a relevance measure for ranking features. Our work aims to develop an understanding of visual model validation which can inform the development of future visualization and machine learning systems.

Model validation is closely related to the viewers' trust in these models and their visualizations. In their state-of-the-art report, Chatzimparmpas et al.\cite{Chatzimparmpas.2020a} summarize the importance of using visualizations to increase trust in machine learning models. In addition to machine learning, the relationship between visual design and trust is an important area of research that should be considered in future work on visual validation\cite{Rogowitz.1996, Peskov.2020, Mayr.2019, Elhamdadi.2022, Dasgupta.2017}.

==> text_initialsubmission/sec-userstudy.tex <==

\section{User Study}
\label{sc:userstudy}

To address our research questions, we first conducted an exploratory pilot study. Based on the results of the pilot, we formulated hypotheses that were subsequently tested in a confirmatory main study. %The derived hypotheses were tested in the main study.

\subsection{Experimental Design}
\label{ssc:expdesign}

The same experimental design and structure was used for both the pilot study and the main study. %Following a between-subject study design, 
We used two \textbf{tasks} to compare the following visual processes:
\begin{itemize}[noitemsep, nolistsep]
    \item \textit{Visual estimation}: Participants had to draw a horizontal line in the plot by hovering over the image with the mouse and clicking on the desired position on the y-axis (\autoref{fig:scat_init}).
    \item \textit{Visual validation}: Participants were shown a scatterplot with a line already drawn and were asked to indicate whether the line was ``too high,'' ``too low,'' or ``about the same'' in relation to their perceived true mean value of the dots (\autoref{fig:scat_line}).
\end{itemize}
We chose a \textbf{between-subject design} of our study for two main reasons: first, it prevents learning effects between the tasks. Second, it reduces the number of trials per participant\cite{Charness.2012}. To maintain consistency, we used the same \textbf{plots} for both the validation and estimation trials.
Each scatterplot, which had dimensions of $100 \times 100$ pixels, contained 100 data points uniformly distributed on the x-axis. The only difference between the two between-subject groups was the lines shown in the validation tasks (see \autoref{fig:scat_init} vs. \autoref{fig:scat_line}).
%the same \textbf{plots} were used for both the validation and estimation trials. Each $[0,100] \times [0,100]$ scatterplot (one scatterplot per trial) consists of 100 data points that are uniformly distributed in the x-axis. The difference in the stimuli of the two between-subject groups arose from the lines shown in the validation tasks. 

For the analysis, we defined the deviation of a line based on the calculation of the confidence interval \textit{(CI)}, which quantifies the \textit{deviation} from the true mean as a proportion of the standard deviation:
\begin{equation}
    \mbox{shown value} = \mbox{true mean} + \mbox{\textit{deviation}} \cdot \mbox{standard deviation}
\end{equation}

%Based on regression calculation, the expected acceptance range of lines lies within the 95\% CI. 
Using regression calculation, the expected acceptance range for lines falls within the 95\% CI.
Given our fixed number of data points and distributions, the 95\% CI is set at a deviation of $0.198$. Thus, all lines with a lower deviation should be considered acceptable.
%In our setting with fixed number of points and data distribution, the 95\% CI is fixed at a deviation of $0.198$. So all lines with lower deviation should be accepted. %This enables us to measure the accuracy of the visual validation. 95\% CI depends only on the z-statistic and the number of points, 

The \textbf{study procedure} began with a training phase, followed by experimental study. Each page of the study interface displayed one trial (i.e., one plot), and participants manually clicked a button to move to the next page so that their answers and response times could be recorded. A display size of at least 13'' was recommended. The order of the trials (i.e., the order in which participants saw different deviations) was randomized to minimize learning effects. At the conclusion of the study, participants were asked to describe their strategies for completing the tasks and rate the task's difficulty on a 5-point Likert scale\cite{Vagias.2006}.
%The \textbf{study process} started with a training phase, then the plots were shown. The study interface contained one trial (i.e., one plot) per page. Participants had to manually click a button to move to the next page so we could record the answers and response time. We recommended a display size of at least 13''. The sorting of the trials (i.e., when participants saw different deviations) was randomized to reduce learning effects. At the end of the study the participants were asked to describe their strategy when solving the tasks and to rate the difficulty of the task on a 5-point Likert scale~\cite{Vagias.2006}. 

\subsection{Pilot Study}
\label{ssc:pilotstudy}

%To get a first intuition about visual validation in general and the differences between the two visual processes, 
To gain an initial understanding of visual validation and its differences from visual estimation, we conducted a pilot study with 12 participants (7 for the validation task and 5 for the estimation task). Each participant answered 30 trials with pseudo-randomized y-coordinates of the scatterplots. The lines shown in the validation task had a random deviation within the range of $\pm [0.0,1.0]$ from  the true mean of the randomly-generated data points.

\smallskip
\noindent \textbf{Results}: The errors in the estimation tasks were roughly normally distributed with $\mu=0.02$ and a maximum deviation of $0.7$. Lines shown in the validation tasks with deviations within the 95\% CI ($dev<0.198$) had acceptance rates of at least 80\%, while every line with $dev>0.198$ had an acceptance rate of at most 30\%. Most participants reported using a ``counting'' strategy to solve the tasks, approximating the number of points above and below a given line.

\input{text/fig-esterror}

\subsection{Main Study}
\label{ssc:mainstudy}

Analysis of the pilot study's results led to the hypotheses:
\begin{itemize}[noitemsep, nolistsep]
    %\item \textbf{H1}: The accuracy of lines getting accepted in visual validation is lower than the accuracy of the visually estimated lines.
    \item \textbf{H1}: The accuracy of visual validation is lower than the accuracy of the visual estimation when perceiving the mean value of points in a scatterplot.
    \item \textbf{H2}: People's critical point between accepting and rejecting a given mean value is close to the boundary of the 95\% CI.
    \item \textbf{H3}: For visual validation, the results differ between positive and negative deviation from the true mean.
\end{itemize}
Study documentation, results, and data generation code are in annex.

\subsubsection{Stimuli Design}
\label{sssc:stimulidesign}

Based on the findings from the pilot study and for matching the distribution assumption of linear regression residuals, the y-coordinates of the points were generated from a normal distribution with a random mean between 30 and 70 and a random standard deviation between 15 and 25. The use of a normal distribution also ensures that all trials are of approximately equal difficulty. Since most participants approximating the median instead of the mean in the pilot study, we ensured that the number of points above and below the true mean differed by at least 10\% to encourage other strategies and discouraging the use of ``bounding boxes''\cite{Yang.2019} as a perceptual proxy. An example scatterplot is shown in \autoref{fig:scat_init}.

The pilot study showed that lines with deviations greater than $0.7$ were consistently rejected. Thus, we used lines with evenly distributed deviations in the range of $\pm [0.0,0.7]$ to determine participants' acceptance threshold. Consistent with previous work\cite{Yang.2019}, logistic regression was chosen to analyze the validation task (see \autoref{sssc:analysis}). A power analysis of the logistic regression of the pilot study indicated that a sample size of at least 50 was necessary to obtain a meaningful model\cite{Motrenko.2014}. Since we aimed to perform logistic regression for each individual participant to check for consistency, the study therefore included 50 trials with 25 lines with a positive and 25 lines with a negative deviation in the validation task.

\input{text/fig-errorcomp}
% \vspace{-15pt}

\subsubsection{Experimental Setting \& Participants}
\label{sssc:expsetting}

To increase the generalizability of our findings, we conducted an online study with two different populations. The first population consisted of 100 individuals who volunteered to participate after seeing advertisements in university lectures and mailing lists. After filtering out 14 participants who failed attention checks, 42 individuals completed the validation task and 44 completed the estimation task.
For the second population, we recruited 90 participants via the crowdsourcing platform Prolific\cite{Prolific}. After filtering for attention checks, 42 individuals completed the validation task and 40 completed the estimation task.
%For the first, 100 people volunteered to participate in the study after being recruited from advertisements in university lectures and mailing-lists. From this participant pool, after filtering out 14 people for not passing the attention questions, 42 people completed the validation and 44 people the estimation tasks. 
%For the second, a total of 90 participants were recruited via the crowdsourcing platform Prolific~\cite{Prolific}. After filtering for the attention questions, 42 people completed the validation and 40 people the estimation tasks.

In both populations, most participants were between 20 and 30 years old (43\% for volunteered, 72\% for crowdsourced) and nearly evenly split between women and men (volunteered: 46\%~F, 50\%~M, 4\%~other; crowdsourced: 47\%~F, 52\%~M, 1\%~other). The level of education and experience with statistical model estimation was slightly higher among the volunteers.


\subsubsection{Analysis}
\label{sssc:analysis}

In the validation task we measured whether participants accepted the displayed line as the true means. 
To ensure comparability with the estimation task results, we transformed the responses to binary results.
%The transformation of the responses to the validation task to binary results was performed to ensure comparability to the estimation task results. 
Logistic regression was then applied to the acceptance rates of the shown lines, which is a technique that has been used in previous work\cite{Yang.2019}.
In the estimation task, we measured whether participants were able to draw (estimate) the true means. 
The estimation errors were measured as the deviation of the lines drawn by the participants.

For statistical testing, we first ran a Shapiro-Wilk test on the given responses and response times to see if they were normally distributed. Although none of the tests were positive, a visual inspection of the acceptance rates and estimation errors suggested that this was due to the large sample size (see \autoref{sssc:results}). Therefore, we used t-tests to compare these results. We used a Kruskal-Wallis test for the response times and a chi-squared test for comparing Likert responses. 

\subsubsection{Results}
\label{sssc:results}

\paragraph{Distribution and Bias}

For both populations, the estimation errors resembled a normal distribution (\autoref{fig:est_error}; $\mu_{volun}<0.01$, $\mu_{crowd}=0.06$), consistent with the regression assumptions. The same is true for the acceptance rates of the lines displayed for validation ($\mu_{volun}=0.01$, $\mu_{crowd}<0.01$). The means of the errors/ acceptance rates being zero indicate that neither of the processes is biased. This finding is supported by a comparison of the acceptance rates for positive and negative deviations from the mean (\autoref{fig:val_error_comp}), which showed no significant difference 
%($\mbox{p-value}_{volun}=0.293$, $\mbox{p-value}_{crowd}=0.721$) \remco{I suggest writing this as: $p_{volun}=0.293$}. 
($\mbox{p}_{volun}=0.293$, $\mbox{p}_{crowd}=0.721$).
This rejects our hypothesis \textbf{H3}.

\input{text/fig-valerrorcomp}

\paragraph{Accuracy of Visual Validation vs. Visual Estimation}

Since both estimation errors and acceptance rates were approximately normally distributed, we considered positive and negative deviations cumulatively as absolute deviations. A comparison of logistic regression for the acceptance rates of the validation task and the cumulative distribution of the estimation errors can be seen in \autoref{fig:comp}. For the volunteered population (\autoref{fig:comp_normal}), 
% accepted models in visual validation were less accurate 
the acceptance threshold for validation was less accurate
than the visually estimated ones; $p<0.0001$, $\mbox{cohensD}=0.35$).

For the crowdsourced population, the difference between the curves was smaller (\autoref{fig:comp_prolific}). While the logistic regressions for validation were almost identical ($p=0.5125$), the estimation errors were higher. Although the accuracy of the visually accepted lines was still lower than the accuracy of the visually estimation lines, the difference was not significant ($p>0.29$).

In summary, our first hypothesis \textbf{H1} is partially accepted.
  
\paragraph{Critical Point of Validation}

\autoref{fig:val_error} shows the raw acceptance rates per deviation and the corresponding logistic regression exemplary for the volunteered population. The inflection points of the logistic regressions correspond by construction to the 50\% acceptance rate. Their values $dev_{volun}=0.217$ and $dev_{crowd}=0.228$ were very close to the boundary of the statistical 95\% CI ($dev=0.198$). Moreover, the critical points of the individuals' logistic regressions resembled a normal distribution near the 95\% CI ($\mu_{volun}=0.223, \mu_{crowd}=0.241$). This indicates that people's perceived visual confidence interval matches the statistical 95\% CI and accepts hypothesis \textbf{H2}.

% To examine individual differences in visual validation, logistic regressions were generated for each participant (see \autoref{sssc:expsetting}) and the resulting inflection points were compared. Although there were some individual differences, they generally follow a normal distribution around the 95\% CI (\autoref{fig:val_inflection}).

\input{text/fig-valerror}

\paragraph{Difficulty and Response Time}

For both populations, no significant difference in response time (\textit{Wilcoxon-test:} volunteered: $\mbox{p-value}=0.9382$, $\mu_{val}=11.3\mbox{sec}$, $\mu_{est}=11.8\mbox{sec}$; crowdsourced: $\mbox{p-value}=0.4968$, $\mu_{val}=10.2\mbox{sec}$, $\mu_{est}=10.5\mbox{sec}$) and reported difficulty (\textit{Chi-squared-test:} volunteered: $\mbox{p-value}=0.2641$, $\mu_{val}=2.76$, $\mu_{est}=3.16$; crowdsourced: $\mbox{p-value}=0.4306$, $\mu_{val}=3.14$, $\mu_{est}=3.22$) was found between the two tasks.  
% This finding suggests that participants do not find one task more difficult than the other, but still perform better overall on estimation over validation.

\paragraph{Self-Reported Strategies}

For visual estimation, most participants derived the mean using a perceptual proxy and ``adjusted it for outliers" (note that there are no true statistical outliers, the participants probably meant points that were a bit off). These perceptual proxies were based on the density of the scatterplot, the median or the distance between the highest and lowest points.

In the visual validation tasks, the majority of the participants validated the line based only on the number of points above and below the line. However, some participants judged based on the perception of the density and structure of the points. The most interesting strategy, however, was that six of the participants first ``estimated [their own] mean and compared it to the shown line.''


%\paragraph{Discussion}
%The results of our study indicate that participants are generally more accurate at performing model estimation than model validation. Moreover, we found that participants are not biased in accepting or rejecting mean lines that have positive or negative deviations from the mean -- and also are capable of perceiving the 95\% CI for the mean height in scatterplots. As a whole, these findings imply that people are quite good at assessing and determining the average of scatterplots.

%Interestingly, we also found that participants do not consider estimation or validation to be significantly more difficult than the other. This result implies that, while participants perform better on estimating the average rather than validating the average, it is not more strenuous for them to perform estimation overall.  

%In summary, the findings of our study suggest that people may perform better at visual model estimation over visual model validation. This result has implications to the design of model visualizations (e.g., that models should not be pre-drawn but estimated by readers); however, how to generalize this implication beyond averages is needed. We discuss future work in the following section.

% \input{text/fig-valinflection}
